Impact-Oriented Contextual Scholar Profiling using Self-Citation Graphs

Quantitatively profiling a scholar's scientific impact is important to modern research society. Current practices with bibliometric indicators (e.g., h-index), lists, and networks perform well at scholar ranking, but do not provide structured context for scholar-centric, analytical tasks such as profile reasoning and understanding. This work presents GeneticFlow (GF), a suite of novel graph-based scholar profiles that fulfill three essential requirements: structured-context, scholar-centric, and evolution-rich. We propose a framework to compute GF over large-scale academic data sources with millions of scholars. The framework encompasses a new unsupervised advisor-advisee detection algorithm, a well-engineered citation type classifier using interpretable features, and a fine-tuned graph neural network (GNN) model. Evaluations are conducted on the real-world task of scientific award inference. Experiment outcomes show that the F1 score of best GF profile significantly outperforms alternative methods of impact indicators and bibliometric networks in all the 6 computer science fields considered. Moreover, the core GF profiles, with 63.6%-66.5% nodes and 12.5%-29.9% edges of the full profile, still significantly outrun existing methods in 5 out of 6 fields studied. Visualization of GF profiling result also reveals human explainable patterns for high-impact scholars.

==> tex/6_discussion.tex <==
\bsec{Discussion}{Dis}

% Discussion
% NLP vs. other fields (result, reason - quality issue): all better in average, but NLP good, even 30% node 30% edge graph much better than existing method; other field not significantly better; impact of data quality (missing citation links); but on other fields with pool data quality, our graph is better than any other networks except DM.
% Graph signatures (mostly full graph better than keynode graph - some fields looks at all papers; for keynode graph, extend edge selection can improve result - for continued work, field look at your key work)
% discussion of outlier field: DM not good for interdisciplinary fields (three outlier features: not significant with other networks, smallest in absolute F1, monotonically decline in extend-edge curve
% implication of graph size comparison in specific sub-fields?

% discussion - superiority of GF

The experiment result implies several findings. First, the proposed method performs better in average than existing methods in representing scholar's impact related to top-level research awards. Yet, the quality of academic data from which we extract GF signatures does matter. In NLP field with the complete ARC data, our method is significantly better than all alternatives. In other fields with incomplete citation links and inaccurate extend-citation inference model, the advantage of GF is mostly insignificant compared with author-level impact indicators and bibliographic networks.

% discussion - GF components

Second, comparing the full graph and core graph signatures, the difference is not clear-cut. Some fields only merit the core papers of a scholar (security), while some others value all papers of the scholar regardless of author order/correspondence (NLP, PL). On extend-type edges, for the NLP field where we have more accurate citation type inference, the extend-type edges are shown to be important as the performance drops more quickly when extend-type edges start to be removed. On other fields, no such conclusion can be drawn as extend-citation inference model is not built with field-specific data. Nevertheless, our smallest core-extend graph signature is proven to be still effective for impact evaluation. In the NLP field, using only 54\% nodes and 15\% edges of the full graph\footnote{This is the 30\% edge setting of core graph, which has 15\% edges of the full graph. Edges unconnected to core papers are removed.}, the core-extend graph achieves significantly better performance than any alternative method. In all the other fields, the performance of core-extend graphs are not significantly lower than its corresponding full graph. We hypothesize that continued, systematic research credited to a scholar could be critical to his/her scientific impact.

% discussion - ???

Finally, we also observe some outliers in the experiment result. The data mining field seems to be different in that GF achieves the lowest F1 score and performs similar to the co-citation network. After examining the dataset, it is found that data mining is an interdisciplinary field where about a half award recipients do not claim it as his/her primary research interests. They may be awarded (ACM fellow) because of the work in other fields, primarily database, machine learning, and AI. Due to the difficulty to identify these scholars, our method in the current design may not be effective for the award inference in interdisciplinary fields.
